Investigating Design Anti-pattern and Design Pattern Mutations and Their Change- and Fault-proneness

During software evolution, inexperienced developers may introduce design anti-patterns when they modify their software systems to fix bugs or to add new functionalities based on changes in requirements. Developers may also use design patterns to promote software quality or as a possible cure for some design anti-patterns. Thus, design patterns and design anti-patterns are introduced, removed, and mutated from one another by developers. Many studies investigated the evolution of design patterns and design anti-patterns and their impact on software development. However, they investigated design patterns or design anti-patterns in isolation and did not consider their mutations and the impact of these mutations on software quality. Therefore, we report our study of bidirectional mutations between design patterns and design anti-patterns and the impacts of these mutations on software change- and fault-proneness. We analyzed snapshots of seven Java software systems with diverse sizes, evolution histories, and application domains. We built Markov models to capture the probability of occurrences of the different design patterns and design anti-patterns mutations. Results from our study show that (1) design patterns and design anti-patterns mutate into other design patterns and/or design anti-patterns. They also show that (2) some change types primarily trigger mutations of design patterns and design anti-patterns (renaming and changes to comments, declarations, and operators), and (3) some mutations of design anti-patterns and design patterns are more faulty in specific contexts. These results provide important insights into the evolution of design patterns and design anti-patterns and its impact on the change- and fault-proneness of software systems.

==> sections/Tables-old.tex <==
\begin{sidewaystable}
\caption{Changes probabilities of anti-patterns and design patterns in ArgoUML}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\begin{center}
\scalebox{0.95}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{2cm}|p{2cm}}
\cline{2-21}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SG & SA & Cm & Cp & FM & De & Ob & PT & Sink \\
\hline
AS& 0.002 & \cellcolor[gray]{0.8}{\textbf{0.388}} & 0.031 & 0.070 & 0.012 & 0.048 & 0.000 & \cellcolor[gray]{0.8}0.113 & 0.033 & 0.048 & 0.031 & 0.000 & 0.005 & 0.038 & 0.000 & \cellcolor[gray]{0.8}0.100 & 0.064 & 0.000 & 0.000 & 0.009 \\
\hline
Bl& 0.003 & 0.008 & \cellcolor[gray]{0.8}{\textbf{0.265}} & 0.058 & \cellcolor[gray]{0.8}0.143 & \cellcolor[gray]{0.8}0.189 & 0.001 & \cellcolor[gray]{0.8}0.142 & 0.052 & 0.079 & 0.004 & 0.010 & 0.000 & 0.010 & 0.000 & 0.000 & 0.021 & 0.000 & 0.000 & 0.009 \\
\hline
CS& 0.004 & 0.053 & 0.070 & \cellcolor[gray]{0.8}{\textbf{0.371}} & 0.053 & 0.068 & 0.001 & \cellcolor[gray]{0.8}0.148 & 0.019 & 0.092 & 0.061 & 0.005 & 0.004 & 0.028 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 \\
\hline
CC& 0.002 & 0.008 & \cellcolor[gray]{0.8}0.186 & 0.052 & \cellcolor[gray]{0.8}{\textbf{0.223}} & \cellcolor[gray]{0.8}0.217 & 0.000 &\cellcolor[gray]{0.8}0.120 & 0.039 & 0.068 & 0.000 & 0.004 & 0.005 & 0.035 & 0.000 & 0.003 & 0.019 & 0.000 & 0.000 & 0.008 \\
\hline
LC& 0.003 & 0.014 & \cellcolor[gray]{0.8}0.193 & 0.054 & \cellcolor[gray]{0.8}0.182 & \cellcolor[gray]{0.8}{\textbf{0.265}} & 0.000 & \cellcolor[gray]{0.8}0.131 & 0.061 & 0.067 & 0.002 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 \\
\hline
LZC& 0.003 & 0.000 & 0.002 & 0.007 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.705}} & 0.008 & 0.000 & 0.072 & \cellcolor[gray]{0.8}0.170 & 0.018 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 \\
\hline
LM& 0.004 & 0.016 & 0.067 & 0.041 & 0.038 & 0.066 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.465}} & 0.058 & \cellcolor[gray]{0.8}0.107 & 0.025 & 0.005 & 0.000 & 0.038 & 0.000 & 0.014 & 0.038 & 0.000 & 0.000 & 0.013 \\
\hline
LP& 0.002 & 0.019 & 0.089 & 0.028 & 0.051 & \cellcolor[gray]{0.8}0.101 & 0.000 & \cellcolor[gray]{0.8}0.162 & \cellcolor[gray]{0.8}{\textbf{0.387}} & 0.080 & 0.016 & 0.001 & 0.000 & 0.004 & 0.000 & 0.002 & 0.012 & 0.000 & 0.000 & 0.009 \\
\hline
MCh& 0.008 & 0.011 & 0.067 & 0.061 & 0.044 & 0.051 & 0.006 & \cellcolor[gray]{0.8}0.176 & 0.037 & \cellcolor[gray]{0.8}{\textbf{0.425}} & 0.052 & 0.007 & 0.000 & 0.007 & 0.000 & 0.000 & 0.006 & 0.000 & 0.000 & 0.024 \\
\hline
RP& 0.009 & 0.008 & 0.005 & 0.056 & 0.001 & 0.000 & 0.036 & 0.069 & 0.011 & 0.065 & \cellcolor[gray]{0.8}{\textbf{0.595}} & 0.058 & 0.000 & 0.024 & 0.000 & 0.001 & 0.035 & 0.000 & 0.000 & 0.026 \\
\hline
SG& 0.006 & 0.019 & 0.049 & 0.027 & 0.029 & 0.044 & 0.014 & 0.061 & 0.003 & 0.039 & \cellcolor[gray]{0.8}0.233 & \cellcolor[gray]{0.8}{\textbf{0.445}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.021 \\
\hline
SA& 0.003 & 0.004 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.980}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 \\
\hline
Cm& 0.002 & 0.036 & 0.003 & 0.025 & 0.038 & 0.000 & 0.000 & 0.041 & 0.004 & 0.006 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.743}} & 0.000 & 0.004 & 0.061 & 0.000 & 0.000 & 0.006 \\
\hline
Cp& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM& 0.002 & 0.013 & 0.000 & 0.000 & 0.004 & 0.000 & 0.000 & 0.013 & 0.003 & 0.006 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.943}} & 0.000 & 0.000 & 0.000 & 0.008 \\
\hline
De& 0.003 & 0.051 & 0.004 & 0.000 & 0.025 & 0.000 & 0.000 & 0.043 & 0.014 & 0.006 & 0.043 & 0.000 & 0.058 & 0.061 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.679}} & 0.000 & 0.000 & 0.009 \\
\hline
Ob& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
PT& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 \\
\hline
\end{tabular}
}
\end{center}
\label{tab:mutation}
%\end{table}
\end{sidewaystable}

\begin{sidewaystable}
%\begin{table}[htbp]
\caption{Changes probabilities of anti-patterns and design patterns in Mylyn}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\begin{center}
\scalebox{0.95}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{2cm}|p{2cm}}
\cline{2-21}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SG &  SA & Cm & Cp & FM & De & Ob & PT & Sink \\
\hline
AS& 0.013& \cellcolor[gray]{0.8}{\textbf{0.323}} & 0.036 & 0.091 & 0.037 & 0.047 & 0.144 & 0.134 & 0.071 & 0.056 & 0.033 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 \\
\hline
Bl& 0.010 & \cellcolor[gray]{0.8}0.209 & \textbf{0.122} & 0.069 & 0.058 & 0.072 & \cellcolor[gray]{0.8}0.211 & 0.108 & 0.055 & 0.039 & 0.004 & 0.010 & 0.000 & 0.019 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.008 \\
\hline
CS& 0.004 & \cellcolor[gray]{0.8}0.221 & 0.026 & \cellcolor[gray]{0.8}{\textbf{0.261}} & 0.031 & 0.040 & 0.126 & 0.104 & 0.072 & 0.061 & 0.029 & 0.000 & 0.000 & 0.019 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 \\
\hline
CC& 0.004 & \cellcolor[gray]{0.8}0.192 & 0.054 & 0.073 & \textbf{0.089} & 0.077 & \cellcolor[gray]{0.8}0.209 & 0.096 & 0.048 & 0.043 & 0.003 & 0.000 & 0.000 & 0.106 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.003 \\
\hline
LC& 0.002 & \cellcolor[gray]{0.8}0.179 & 0.043 & 0.066 & 0.053 & \textbf{0.105} & \cellcolor[gray]{0.8}0.174 & 0.084 & 0.041 & 0.027 & 0.001 & 0.001 & 0.000 & \cellcolor[gray]{0.8}0.215 & 0.002 & 0.002 & 0.000 & 0.001 & 0.001 & 0.004 \\
\hline
LZC& 0.106 & 0.131 & 0.035 & 0.041 & 0.038 & 0.052 & \textbf{0.048} & 0.118 & 0.106 & 0.085 & \cellcolor[gray]{0.8}0.153 & 0.005 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.075 \\
\hline
LM& 0.007 & \cellcolor[gray]{0.8}0.175 & 0.026 & 0.052 & 0.025 & 0.033 & 0.142 & \textbf{0.337} & 0.076 & 0.059 & 0.035 & 0.001 & 0.000 & 0.017 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 \\
\hline
LP& 0.003 & 0.145 & 0.007 & 0.043 & 0.007 & 0.016 & \cellcolor[gray]{0.8}0.214 & 0.113 & \textbf{0.114} & 0.007 & 0.005 & 0.001 & 0.000 & \cellcolor[gray]{0.8}0.313 & 0.003 & 0.002 & 0.000 & 0.000 & 0.001 & 0.002 \\
\hline
MCh& 0.013 & \cellcolor[gray]{0.8}0.189 & 0.018 & 0.091 & 0.021 & 0.023 & \cellcolor[gray]{0.8}0.325 & \cellcolor[gray]{0.8}0.151 & 0.031 & \textbf{0.075} & 0.022 & 0.000 & 0.000 & 0.026 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.009 \\
\hline
RP& 0.006 & 0.126 & 0.001 & 0.033 & 0.001 & 0.001 & \cellcolor[gray]{0.8}0.425 & 0.071 & 0.016 & 0.021 & \textbf{0.107} & 0.000 & 0.000 & \cellcolor[gray]{0.8}0.182 & 0.002 & 0.001 & 0.000 & 0.000 & 0.000 & 0.005 \\
\hline
SG& 0.011 & 0.087 & 0.011 & 0.017 & 0.017 & 0.041 & \cellcolor[gray]{0.8}0.369 & 0.081 & 0.109 & 0.011 & 0.011 & \cellcolor[gray]{0.8}{\textbf{0.158}} & 0.000 & 0.064 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 \\
\hline
SA& 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.999}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cm& 0.000 & 0.000 & 0.035 & 0.017 & 0.095 & \cellcolor[gray]{0.8}0.216 & 0.000 & 0.016 & \cellcolor[gray]{0.8}0.301 & 0.042 & 0.173 & 0.072 & 0.003 & \cellcolor[gray]{0.8}{\textbf{0.448}} & 0.003 & 0.003 & 0.011 & 0.001 & 0.018 & 0.000 \\
\hline
Cp& 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.997}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.000 & 0.003 & 0.002 & 0.002 & 0.001 & 0.000 & 0.004 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.980}} & 0.003 & 0.000 & 0.000 & 0.000 \\
\hline
De& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.061 & 0.000 & 0.006 & \cellcolor[gray]{0.8}{\textbf{0.927}} & 0.000 & 0.000 & 0.000 \\
\hline
Ob& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.996}} & 0.000 & 0.000 \\
\hline
PT& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.995}} & 0.000 \\
\hline
\end{tabular}
}
\end{center}
\label{tab:mylynmutation}
%\end{table}
\end{sidewaystable}

\begin{sidewaystable}
%\begin{table}[htbp]
\caption{Changes probabilities of anti-patterns and design patterns in Rhino}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\begin{center}
\scalebox{0.95}{
\begin{tabular}
%\begin{sidewaystable}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\cline{2-21}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SG &  SA & Cm & Cp & FM & De & Ob & PT & Sink \\
\hline
AS& 0.006 & \cellcolor[gray]{0.8}\textbf{0.191} & 0.000 & 0.101 & 0.097 & 0.097 & 0.000 & \cellcolor[gray]{0.8}0.151 & 0.101 & \cellcolor[gray]{0.8}0.208 & 0.035 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.007 \\
\hline
Bl& 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.999} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 \\
\hline
CS& 0.011 & 0.038 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.335} & 0.070 & 0.008 & 0.093 & 0.070 & \cellcolor[gray]{0.8}0.235 & 0.048 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 \\
\hline
CC& 0.001 & 0.035 & 0.000 & 0.075 & \cellcolor[gray]{0.8}\textbf{0.236} & \cellcolor[gray]{0.8}0.238 & 0.000 & 0.108 & 0.119 & \cellcolor[gray]{0.8}0.171 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.002 \\
\hline
LC& 0.001 & 0.035 & 0.000 & 0.073 & \cellcolor[gray]{0.8}0.225 & \cellcolor[gray]{0.8}\textbf{0.271} & 0.000 & 0.104 & 0.114 & \cellcolor[gray]{0.8}0.162 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 \\
\hline
LZC& 0.054 & 0.000 & 0.000 & 0.045 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.652} & 0.000 & 0.000 & 0.000 & 0.119 & 0.060 & 0.000 & 0.020 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.066 \\
\hline
LM& 0.010 & 0.044 & 0.000 & 0.076 & 0.076 & 0.079 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.336} & 0.107 & \cellcolor[gray]{0.8}0.226 & 0.021 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.014 \\
\hline
LP& 0.007 & 0.036 & 0.000 & 0.075 & 0.119 & 0.119 & 0.000 & 0.138 & \cellcolor[gray]{0.8}\textbf{0.260} & \cellcolor[gray]{0.8}0.214 & 0.019 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 \\
\hline
MCh& 0.008 & 0.043 & 0.000 & 0.138 & 0.079 & 0.081 & 0.000 & 0.141 & 0.101 & \cellcolor[gray]{0.8}\textbf{0.362} & 0.029 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.011 \\
\hline
RP& 0.022 & 0.045 & 0.000 & 0.121 & 0.035 & 0.035 & 0.035 & 0.069 & 0.070 & 0.111 & \cellcolor[gray]{0.8}\textbf{0.363} & 0.059 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.028 \\
\hline
SG& 0.037 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.111 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}0.277 & \cellcolor[gray]{0.8}\textbf{0.527} & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.045 \\
\hline
SA& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{1} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
Cm& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.997} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
Cp& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{1} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{1} & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
De& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.998} & 0.000 & 0.000 & 0.000 \\
\hline
Ob& 0.000 & 0.002 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.004 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{0.990} & 0.000 & 0.000\\
\hline
PT& 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}\textbf{1} & 0.000\\
\hline
\end{tabular}
}
\end{center}
\label{tab:rhinomutation}
%\end{table}
\end{sidewaystable}


==> sections/Tables.tex <==
%Eclipse
\begin{table*}
\caption{Change probabilities of anti-patterns and design patterns in Eclipse IDE}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.8}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.013 & \cellcolor[gray]{0.8}{\textbf{0.972}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.015 \\
\hline
Bl & 0.007 & \cellcolor[gray]{0.8}{\textbf{0.27}} & \cellcolor[gray]{0.8}{\textbf{0.447}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.277}} \\
\hline
CS & 0.001 & 0.000 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.993}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 \\
\hline
CC & 0.000 & 0.000 & 0.000 & 0.012 & \cellcolor[gray]{0.8}{\textbf{0.973}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.5}} & \cellcolor[gray]{0.8}{\textbf{0.5}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & \cellcolor[gray]{0.982}{\textbf{0.859}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 \\
\hline
LM & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.024 & \cellcolor[gray]{0.8}{\textbf{0.95}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.025 \\
\hline
LP & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.009 & \cellcolor[gray]{0.8}{\textbf{0.966}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.025 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.273}} & \cellcolor[gray]{0.8}{\textbf{0.455}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.273}} \\
\hline
SC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline 
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.876}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.049 & 0.000 & 0.002 & 0.05 \\
\hline
Cm & 0.000 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.668}} & 0.091 & 0.09 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.141}} \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.042 & \cellcolor[gray]{0.8}{\textbf{0.169}} & \cellcolor[gray]{0.8}{\textbf{0.665}} & 0.076 & 0.000 & 0.000 & 0.000 & 0.042 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.892}} & \cellcolor[gray]{0.8}{\textbf{0.107}} & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.020 & \cellcolor[gray]{0.8}{\textbf{0.966}} & 0.014 \\
\hline
\end{tabular}
}
\label{tab:EclipseMarkov}
\end{table*}


\begin{table*} [ht]
\caption{Change probabilities of anti-patterns and design patterns in Nuxeo}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.8}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.014 & \cellcolor[gray]{0.8}{\textbf{0.969}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.017 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
Bl & 0.003 & \cellcolor[gray]{0.8}{\textbf{0.283}} & \cellcolor[gray]{0.8}{\textbf{0.417}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.297}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
CS & 0.002 & 0.000 & 0.008 & \cellcolor[gray]{0.8}{\textbf{0.982}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
CC & 0.001 & 0.000 & 0.000 & 0.040 & \cellcolor[gray]{0.8}{\textbf{0.912}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.047 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.048 & \cellcolor[gray]{0.8}{\textbf{0.910}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.042 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LM & 0.001 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.028 & \cellcolor[gray]{0.8}{\textbf{0.937}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.030 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LP & 0.000 & 0.001 & 0.000 & 0.006 & 0.000 & 0.000 & 0.002 & 0.017 & \cellcolor[gray]{0.8}{\textbf{0.946}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.028 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SC & 0.012 & 0.000 & 0.000 & 0.012 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.067 & \cellcolor[gray]{0.8}{\textbf{0.824}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.85 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline 
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.019 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.133}} & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.105}} & \cellcolor[gray]{0.8}{\textbf{0.760}} & 0.000 \\
\hline
\end{tabular}
}
\label{tab:Nuxeomarkov}
\end{table*}


\begin{table*}
\caption{Change probabilities of anti-patterns and design patterns in Ovirt}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.018 & \cellcolor[gray]{0.8}{\textbf{0.971}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.011\\
\hline
Bl & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.299}} & \cellcolor[gray]{0.8}{\textbf{0.394}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.308}}\\
\hline
CS & 0.006 & 0.000 & 0.003 & \cellcolor[gray]{0.8}{\textbf{0.982}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 \\
\hline
CC & 0.000 & 0.000 & 0.000 & 0.012 & \cellcolor[gray]{0.8}{\textbf{0.975}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.013 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.998}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 \\
\hline
LM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & \cellcolor[gray]{0.8}{\textbf{0.977}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.011 \\
\hline
LP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & \cellcolor[gray]{0.8}{\textbf{0.969}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.022 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.082 & \cellcolor[gray]{0.8}{\textbf{0.857}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.061 \\
\hline
SC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline 
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.019 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.097}} & \cellcolor[gray]{0.8}{\textbf{0.798}} & \cellcolor[gray]{0.8}{\textbf{0.103}} \\
\hline
\end{tabular}
}
\label{tab:Ovirtmarkov}
\end{table*}

\begin{table*} 
\caption{Change probabilities of anti-patterns and design patterns in Matsim}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.066 & \cellcolor[gray]{0.8}{\textbf{0.893}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.040 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
Bl & 0.003 & \cellcolor[gray]{0.8}{\textbf{0.372}} & \cellcolor[gray]{0.8}{\textbf{0.279}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.346}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
CS & 0.025 & 0.000 & 0.037 & \cellcolor[gray]{0.8}{\textbf{0.9}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.038 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
CC & 0.004 & 0.001 & 0.002 & 0.075 & \cellcolor[gray]{0.8}{\textbf{0.848}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.069 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.1}} & \cellcolor[gray]{0.8}{\textbf{0.831}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.066 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LM & 0.003 & 0.001 & 0.002 & 0.013 & 0.000 & 0.000 & 0.063 & \cellcolor[gray]{0.8}{\textbf{0.86}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.059 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LP & 0.003 & 0.000 & 0.003 & 0.013 & 0.000 & 0.000 & 0.007 & 0.034 & \cellcolor[gray]{0.8}{\textbf{0.887}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.053 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.021 & \cellcolor[gray]{0.8}{\textbf{0.596}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.193}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SC & 0.026 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.038 & \cellcolor[gray]{0.8}{\textbf{0.834}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.099}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline 
SG & 0.000 & 0.000 & 0.000 & 0.091 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.182}} & \cellcolor[gray]{0.8}{\textbf{0.455}} & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.273}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.546}} & 0.000 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.272}} & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.141}} & 0.000 & 0.030 & 0.000 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.030 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.371}} & 0.075 & \cellcolor[gray]{0.8}{\textbf{0.387}} & \cellcolor[gray]{0.8}{\textbf{0.117}} & 0.012 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.037 & 0.044 & \cellcolor[gray]{0.8}{\textbf{0.850}} & 0.061 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.001 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.036 & 0.074 & \cellcolor[gray]{0.8}{\textbf{0.825}} & 0.059 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.049 & \cellcolor[gray]{0.8}{\textbf{0.912}} & 0.034 & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.028 & 0.000 & 0.000 & 0.009 & \cellcolor[gray]{0.8}{\textbf{0.962}} & 0.000 \\
\hline
\end{tabular}
}
\label{tab:MatsimMarkov}
\end{table*}

\begin{table*} 
\caption{Change probabilities of anti-patterns and design patterns in ApacheSolr}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bl & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.321}} & \cellcolor[gray]{0.8}{\textbf{0.365}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.313}} \\
\hline
CS & 0.000 & 0.000 & 0.009 & \cellcolor[gray]{0.8}{\textbf{0.983}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 \\
\hline
CC & 0.000 & 0.000 & 0.000 & 0.033 & \cellcolor[gray]{0.8}{\textbf{0.93}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.037 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.072 & \cellcolor[gray]{0.8}{\textbf{0.859}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.069 \\
\hline
LM & 0.000 & 0.000 & 0.001 & 0.002 & 0.000 & 0.000 & 0.033 & \cellcolor[gray]{0.8}{\textbf{0.928}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.036 \\
\hline
LP & 0.000 & 0.001 & 0.000 & 0.008 & 0.000 & 0.000 & 0.007 & 0.079 & \cellcolor[gray]{0.8}{\textbf{0.779}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.125 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.088 & \cellcolor[gray]{0.8}{\textbf{0.84}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.072 \\
\hline
SC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.013 & 0.000 &  \cellcolor[gray]{0.8}{\textbf{0.981}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 \\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.963}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.000 & 0.027 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & \cellcolor[gray]{0.8}{\textbf{0.874}} & 0.005 & 0.000 & 0.000 & 0.000 & 0.092 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.996}} & 0.000 & 0.000 & 0.000 & 0.004 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.007 & \cellcolor[gray]{0.8}{\textbf{0.981}} & 0.012 \\
\hline
\end{tabular}
}
\label{tab:SolrMarkov}
\end{table*}


\begin{table*} 
\caption{Change probabilities of anti-patterns and design patterns in ApacheIgnite}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bl & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.375}} & \cellcolor[gray]{0.8}{\textbf{0.33}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.295}} \\
\hline
CS & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 &  0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
CC & 0.000 & 0.000 & 0.000 & 0.053 & \cellcolor[gray]{0.8}{\textbf{0.905}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.042 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.015 & \cellcolor[gray]{0.8}{\textbf{0.97}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.015 \\
\hline
LM & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.000 & 0.045 & \cellcolor[gray]{0.8}{\textbf{0.905}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.047 \\
\hline
LP & 0.000 & 0.000 & 0.000 & 0.009 & 0.000 & 0.000 & 0.006 & 0.051 & \cellcolor[gray]{0.8}{\textbf{0.851}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.081 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.976}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.000 & 0.018 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & \cellcolor[gray]{0.8}{\textbf{0.994}} & 0.003 \\
\hline
\end{tabular}
}
\label{tab:IgniteMarkov}
\end{table*}
%\end{sidewaystable}

\begin{table*}
\caption{Change probabilities of anti-patterns and design patterns in Mule}
\setlength\tabcolsep{0.08cm}% let LaTeX calculate intercolumn whitespace
\scriptsize
\centering
\scalebox{0.75}{
\begin{tabular}
{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|p{0.5cm}|p{0.5cm}}
\cline{2-24}
\multicolumn{1}{l|}{}& Source & AS & Bl & CS & CC & LC & LZC & LM & LP & MCh & RP & SC & SG & SA & Bu & Cm & Cp & FM & De & Ob & PT & Si & Sink \\
\hline
AS & 0.032 & \cellcolor[gray]{0.8}{\textbf{0.937}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.030 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
Bl & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.313}} & \cellcolor[gray]{0.8}{\textbf{0.313}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.374}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
CS & 0.003 & 0.000 & 0.006 & \cellcolor[gray]{0.8}{\textbf{0.963}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.028 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
CC & 0.001 & 0.000 & 0.000 & 0.071 & \cellcolor[gray]{0.8}{\textbf{0.843}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.084 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LZC & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.030 & \cellcolor[gray]{0.8}{\textbf{0.946}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.024 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LM & 0.000 & 0.000 & 0.000 & 0.010 & 0.000 & 0.000 & 0.039 & \cellcolor[gray]{0.8}{\textbf{0.907}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.044 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
LP & 0.000 & 0.000 & 0.000 & 0.014 & 0.000 & 0.000 & 0.009 & \cellcolor[gray]{0.8}{\textbf{0.115}} & \cellcolor[gray]{0.8}{\textbf{0.676}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.186}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
MCh & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
RP & 0.000 & 0.000 & 0.000 & 0.033 & 0.000 & 0.000 & 0.067 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.233}} & \cellcolor[gray]{0.8}{\textbf{0.233}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.433}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
SC & \cellcolor[gray]{0.8}{\textbf{0.096}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.074 & \cellcolor[gray]{0.8}{\textbf{0.649}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.181}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline 
SG & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.053 & \cellcolor[gray]{0.8}{\textbf{0.947}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000\\
\hline
SA & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Bu & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.708}} & 0.000 & 0.001 & \cellcolor[gray]{0.8}{\textbf{0.152}} & 0.000 & 0.067 & 0.000 & 0.065 & 0.000 \\
\hline
Cm & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.019 & 0.000 & \cellcolor[gray]{0.8}{\textbf{0.687}} & \cellcolor[gray]{0.8}{\textbf{0.096}} & \cellcolor[gray]{0.8}{\textbf{0.193}} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
Cp & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.058 & \cellcolor[gray]{0.8}{\textbf{0.882}} & 0.054 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
FM & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.000 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.042 & 0.087 & \cellcolor[gray]{0.8}{\textbf{0.764}} & \cellcolor[gray]{0.8}{\textbf{0.099}} & 0.000 & 0.000 & 0.000 & 0.000 \\
\hline
De & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 & \cellcolor[gray]{0.8}{\textbf{0.971}} & 0.013 & 0.000 & 0.000 & 0.000 \\
\hline
Ob & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.024 & 0.024 & \cellcolor[gray]{0.8}{\textbf{0.951}} & 0.000 & 0.000 & 0.000 \\
\hline
PT & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & \cellcolor[gray]{0.8}{\textbf{1}} & 0.000 & 0.000 \\
\hline
Si & 0.000 & 0.000 & 0.000 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.029 & 0.000 & 0.000 & 0.006 & \cellcolor[gray]{0.8}{\textbf{0.964}} & 0.000 \\
\hline
\end{tabular}
}
\label{tab:Mulemarkov}
\end{table*}


